DMR API: Improving cluster productivity by turning applications into malleable

Adaptive workloads can change on--the--fly the configuration of their jobs, in terms of number of processes. In order to carry out these job reconfigurations, we have designed a methodology which enables a job to communicate with the resource manager and, through the runtime, to change its number of MPI ranks. The collaboration between both the workload manager---aware of the queue of jobs and the resource allocation---and the parallel runtime---able to transparently handle the processes and the program data---is crucial for our throughput-aware malleability methodology. Hence, when a job triggers a reconfiguration, the resource manager will check the cluster status and return an action: an expansion, if there are spare resources; a shrink, if queued jobs can be initiated; or none, if no change can improve the global productivity. In this paper, we describe the internals of our framework and how it is capable of reducing the global workload completion time along with providing a smarter usage of the underlying resources. For this purpose, we present a thorough study of the adaptive workloads processing by showing the detailed behavior of our framework in representative experiments and the low overhead that our reconfiguration involves.

==> text/abstract.tex <==
\begin{abstract}

%Process migration within nodes in cluster can suppose an extra in adaptivity to the new emerging lines in supercomputation.
%From a better managing of resources by moving their workload or consolidating it in specific nodes; to the dealing with heterogeneous infrastructure that an application might not be using during its whole execution; going through the resiliency that migration is able to provide.

%However, the migration of processes implies a deep knowledge of the cluster status in order to assign the most appropriate resource to each job. Hence, the combination of the migration technology with a RMS (Resource Manager System) aware of the cluster status seems to be a good outlet for automatic reconfiguration of jobs in HPC facilities.

%Moreover, in terms of HPC, jobs are launched to a job queue with a given requirements of walltime, memory, nodes... 
%These requirements remain constant during the whole execution ignoring the status of the queue.
%At this point is where our idea can make a difference when talking of throughput turning them malleable.

%Thus, the adoption of new programming models capable of dealing with heterogeneity in HPC infrastructures has brought new possibilities unthinkable several years ago. Thanks to the runtimes that many models use implicitly, the execution of an application remains governed by them in order to increase their performance and the throughput. In this work, we have paid attention to this last measure.

%Application malleability is crucial to
%attain high resource utilization. Non-malleable jobs in a cluster use
%a static amount of resources, regardless of their computational
%stage and the available resources in the facility. 
In this paper we introduce a methodology for dynamic job reconfiguration driven by the programming model runtime in collaboration with the global resource manager.  
We improve the system throughput by exploiting malleability techniques (in terms of number of MPI ranks) through the reallocation of resources assigned to a job during its execution.
In our proposal, the OmpSs runtime reconfigures the number of MPI ranks during the execution of an application in cooperation with the Slurm workload manager. 
In addition, we take advantage of OmpSs offload semantics to allow application developers deal with data redistribution. 
By combining these elements a job is able to expand itself in order to exploit idle nodes or be shrunk if other queued jobs could be
initiated. This novel approach adapts the system workload in order to increase the throughput as well as make a smarter use of the underlying resources.
%Experimental results with both synthetic benchmarks and applications
%demonstrate the notable increase in throughput brought by this approach.
Our experiments demonstrate that this approach can reduce the total execution time of a practical workload by more than 40\% while reducing the amount of resources by 30\%.
\end{abstract}


==> text/background.tex <==
\section{Background}
\label{sec:background}
In this section we introduce the basic components of our
proposal: the programming model framework and the RMS. 
\subsection{The OmpSs Programming Model and its Framework}
OmpSs is a directive-based programming model which leverages asynchronous
parallelism by determining the data dependencies among tasks. 
The programmer is in charge of specifying the size and access mode of
the tasks' data buffers, depending on whether these will be read, written, or
both (annotated as ``in'', ``out'', and ``inout'', respectively).
The OmpSs offload semantics~\cite{Sainz2015} enable
delegating tasks to remote compute nodes. This extension of OmpSs was initially
designed to support the execution of tasks on the most
architecturally-appropriate node in heterogeneous clusters.

The \texttt{Mercurium} source-to-source compiler interprets the
directives in order to generate the appropriate calls to the
\texttt{Nanos++} runtime system.
The latter is a modular, extensible, and portable runtime for
parallel and distributed systems that currently supports OmpSs as well as OpenMP.


\subsection{The Slurm Workload Manager}
\label{back:slurm}
Slurm runs a daemon on each compute node of a cluster that communicates with a controller daemon in the management node.
Slurm manages nodes and their resources; partitions (sets of nodes); 
jobs or allocations of resources assigned to a user; 
and job steps, which are sets of tasks within a job. 
A submitted job is pushed into a priority-aware queue associated
with a cluster partition. 

The modular design of Slurm eases its extension by loading new
plug-ins for non-core functionality such as accounting, scheduling
policy, authentication, generic resources, or resource selection.
Moreover, it exposes an external API that may be used by external
software agents.
Furthermore, by using its API, Slurm provides a job resize mechanism driven by the user, following the next steps:

\paragraph{Job A has to be expanded}
\begin{enumerate}
\item Submit a new job B with a dependency on the initial job A.
Job B requests the number of nodes NB to be added to job A.
\item Update job B, setting its number of nodes to~0.
This produces a set of NB allocated nodes which are not attached to any job.
\item Cancel job B.
\item Update job A and set its number of nodes to NA+NB.
\end{enumerate}

\paragraph{Job A has to be shrunk}
\begin{enumerate}
\item Update job A, setting the new number of nodes to the final size (NA is updated).
\end{enumerate}

After these steps, Slurm's \textit{environment variables} for job A are
updated. 
These commands have no effect on the status of the running job, and the user remains responsible for any process malleability and data redistribution.

Our throughput-oriented malleability framework builds upon this feature.
%For this purpose, we have developed a resource selection plug-in responsible for reconfiguration decisions. %based on the existing plug-in \texttt{select/linear}.
%This plug-in establishes a communication between the RMS and the extended
%Nanos++ runtime, in order to send the optimal resizing action for overall
%system throughput optimization.

%Hence, we have chosen Slurm not only because it is one of the most adopted RMS in HPC facilities~\cite{top500}, but also because its extensibility.



==> text/exp-preliminary.tex <==
\section{Preliminary Study}
\label{sec:preliminary}
In this section we present an in-depth analysis of the framework's features using synthetic flexible jobs.
In order to test thoroughly the features of our solution, we performed 4 different experiments comprising: synchronous and asynchronous scheduling, heterogeneous workload, and micro-steps.

\subsection{Testbed}
For this study we only used the FS application; 
we generated several workloads of different size (number of \texttt{jobs}), assigning up to 20 nodes to each job (the number of available nodes in this experiment) with the parameter \texttt{job size}; 
the maximum \texttt{runtime} was set to 60 seconds for each step; 
and the average \texttt{arrival} time was 10 seconds.
Table~\ref{tab:apps-conf} details the rest of the FS parameters for the reconfigurations.
The array was determined to have 1~GB of data transferred in each iteration.
Furthermore, by not giving a \texttt{preferred} value the RMS has more freedom to reallocate resources.

\begin{table}
\caption{Configuration parameters for the applications}
\label{tab:apps-conf}
\centering
\ra{1} 
%\resizebox{\linewidth}{!}{%
\begin{tabular}{rccccc} 
\toprule
& & \multicolumn{3}{c}{Number of Processes} & \\ \cline{3-5}
Application & Iterations &  Minimum & Maximum & Preferred & Scheduling period\\ \midrule
FS & 25 & 1 & 20 & - & -\\
CG & 10000 & 2 & 32 & 8 & 15 seconds\\
Jacobi & 10000 & 2  & 32 & 8 & 15 seconds\\
N-body & 25 & 1 & 16 & 1 &  -\\
\bottomrule
\end{tabular}%}
\end{table}

\subsection{Synchronous Reconfiguration Scheduling} 
\begin{figure}%[htp]
  \centering
\includegraphics[clip,width=0.75\columnwidth, trim={2.8cm 4.75cm 2.8cm 4cm}]{images/syncExecTime.pdf}
\caption{Comparison between fixed and flexible workloads with different number of jobs.}\label{fig:syncExecTime}
\end{figure}

\begin{figure}%[ht]
  \centering
  \includegraphics[clip,width=0.75\columnwidth]{images/sync10-R-both.png}
  \caption{Evolution in time for the 10-job workload.}\label{fig:sync10}
    %\vspace{-0.5cm}
\end{figure}

\begin{figure}%[ht]
  \centering
\stackinset{l}{2.9in}{b}{0.25in}{\rotatebox{90}{\rule{2.85in}{1.25pt}}}{%
  \includegraphics[clip,width=0.75\columnwidth]{images/sync25-R-both.png}}
  \caption{Evolution in time for the 25-job workload.}\label{fig:sync25}
    %\vspace{-0.5cm}
\end{figure}

For the first test, we launched workloads of different sizes in terms of number of jobs.
Figure~\ref{fig:syncExecTime} depicts the execution time for this experiment.
Each workload has both a fixed as well as a flexible version.
The line ``Gain'' in that chart indicates the reduction of the execution time (in \%) attained by the flexible workload with respect to the fixed workload.

Except for the 10-job workload, we can appreciate a gain in the interval 10-15\% for the execution time,
though the benefit decreases as the workload grows.
Nonetheless, this occurs because we are evaluating a finite workload.
Under these conditions, the scheduler is able to backfill jobs and fulfill resources, but malleability cannot bring a higher resource utilization.
In a more realistic scenario, involving a much larger workload,  the throughput is always higher for the flexible workloads.
For instance, bottom plots in Figures~\ref{fig:sync10} and~\ref{fig:sync25} show that the productivity attained by the flexible workload is always higher than that offered by the fixed workload.

Figure~\ref{fig:sync10} reports an almost-full allocation of resources during the flexible execution, exposing that the remarkable gain is due to the augment in resource usage.

In contrast, Figure~\ref{fig:sync25} depicts the behavior of a workload of 25 jobs, for which we observe a narrower gain.
The problem here arises on the last job (LJ) just in the vertical black line in that figure.
Specifically, in that instant LJ is using 4 nodes while the penultimate job (PJ) before completion,  
owns the rest of resources.
When PJ finishes, 16 nodes are released, but until the next check, LJ cannot be expanded.
At that point, the scheduler decides to expand the job to its maximum, in this experiment 16 nodes.
At the end of the timeline, no more jobs can use the spare resources.
This is the same situation that appears in the fixed workload.
The consequence is that there is no further improvement, 
as the flexible policy had already obtained the gain from the first reallocation of resources.

\subsection{Asynchronous Reconfiguration Scheduling} 
\label{subsubsec:async}

\begin{figure}%[ht]
\centering
\begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[clip,width=0.75\columnwidth]{images/async10-R-both.png}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[black,thick,rounded corners] (0.45,0.975) rectangle (0.6,0.575);
        \draw[black,thick,rounded corners] (0.675,0.975) rectangle (0.8,0.575);
    \end{scope}
\end{tikzpicture}
\caption{Asynchronous scheduling of the 10-job workload.}\label{fig:async10}
\end{figure}

\begin{figure}%[htp]
\centering
  \includegraphics[clip,width=0.75\columnwidth,  trim={2.5cm 10.35cm 2.5cm 11.5cm}]{images/asyncExecTime.pdf}
\caption{Comparison between fixed and flexible workloads using asynchronous selection of action.}\label{fig:asyncExecTime}
\end{figure}

In this test we evaluated the asynchronous version of the scheduling.
Again, we compare a fix workload and its flexible counterpart, but now the decision is made asynchronously.
Here, we remind that the asynchronous scheduling takes a decision in a specific step but the action takes place in the next step.
In the meantime, the status of the system may change. 
Therefore, the conditions found when the action is applied in the next step might not be the same that were present when the RMS decided the future action.
In this situation, enforcing outdated actions may result in an inefficient use of resources.
 
Let us analyze the effect of adopting outdated decisions for the asynchronous scheduling in the 10-job workload.
In this example the flexible workload performs worse than the fixed execution.
We can explain the cause analyzing Figure~\ref{fig:async10}. 
If we focus on the resource allocation evolution (top of Figure~\ref{fig:async10}), two relevant gaps can be identified between seconds 2000-3000 and 3000-4000.
At the beginning of the first gap in Figure~\ref{fig:async10}, there are 3 jobs in execution that occupy a total of 19 nodes:
one (J1) with 16, one (J2) with 2, and a last one (J3) with 1.
Moreover, the RMS has decided to expand J3 to 2 nodes in the next step.
Now, J1 is finished, leaving the other 2 active jobs using 3 nodes (J3 has not expanded yet).
J2 is resolved to expand and acquires 16 nodes (around second 2500).
J3 experiences a longer step, carrying out its pending action of expanding to 2, yielding an overall of 18 allocated nodes.
If J3 had checked the resources at that moment, it would have been expanded to 4 nodes, but the asynchronous scheduling was negotiated earlier, when the conditions were different.
In addition to realizing the expansion, the scheduler decides that J3 will expand to 4 nodes in the next step.

The beginning of the second gap indicates the completion of J2.
A few seconds later J3 expands to 4 nodes (instead of doing it to 16 if the scheduling had been synchronous).

Despite the lack of good results for small workloads, the larger workload completion times reveal a higher gain.
In that type of situation the malleability overcomes the initial problem described above.

As we did in the synchronous benchmark (Figure~\ref{fig:syncExecTime}), if we dismiss the small executions (10-to-50-job workloads), we can observe around a 6\%-gain, with the improvement decreasing as we add more jobs to the workload.

 \begin{table}
 \caption{Cluster and job measures of the 400-job workloads.}
 \label{tab:aggregated}
 \centering
 %\resizebox{\linewidth}{!}{
 \begin{tabular}{lrccc}
 \toprule
 \multicolumn{2}{c}{Cluster Measures} & Fixed & Synchronous & Asynchronous \\ \midrule
\multirow{2}{*} {Resources utilization} & Avg. (\%) & 83.607& 93.909& 86.687 \\
 & Std. (\%) & 5.353&1.012 &  8.735 \\ \midrule
 \multicolumn{2}{c}{Per Job Measures} & Fixed & Synchronous & Asynchronous \\ \midrule
\multirow{2}{*} {Waiting time gain} & Avg. (\%) & - &  27.980& 30.575\\
 & Std. (\%) & -& 12.124 & 17.282\\
\multirow{2}{*} {Execution time gain} & Avg. (\%) & - &-58.482 & -97.294 \\
 & Std. (\%) &- & 26.731 & 34.378\\
\multirow{2}{*} {Completion time gain} & Avg. (\%) & - & 12.786&  7.799\\
 & Std. (\%) & -& 4.083& 5.548\\
 \bottomrule
 \end{tabular}%}
 \end{table}
 
 In Table~\ref{tab:aggregated} we compare both modes, synchronous and asynchronous, in more detail analyzing their performance at cluster level and at job level.
 The most remarkable aspect here is that the synchronous scheduling occupies almost all the resources during the complete executions (the low standard deviation reveals that the mean value is barely unchanged for all the sizes).
 Moreover, the asynchronous mode still presents a higher utilization rate than the configuration without flexible jobs.
 However, the high standard deviation means that the utilization is not as regular as in the synchronous case.
 In fact, this result hides a low average utilization for small workloads (as we already reported in this subsection, the small workloads performed worst) compared with a high  average for large workloads, similar to the synchronous scenario.
  
 The three last columns offer information about timing measures: the wait-time of a job before entering execution, the execution time of the job, and the difference of time from the job submission to its finalization (completion).
 Malleability provides an important reduction of the wait-time in both modes for all the sizes.
 This is because the resource manager can shrink a job in execution in favor of a queued one.
 
 With respect to the execution time, we experience a high degradation in the performance of each individual job.
 For the synchronous scheduling, the negative gain of around a 50\% is closely related to the fact that the application scales linearly.
 Thus, halving the resources produces a proportional reduction of the performance.
 In the asynchronous scenario, the degradation is even worse due to the drawbacks discussed in~\ref{subsubsec:async}.
 The high standard deviation means that not all the jobs perform so bad; in fact, the jobs in the small workloads are the most affected instances (as showed in Figure~\ref{fig:asyncExecTime}).
 
 Finally, the global job time (completion time) places malleability in a good position, especially the synchronous scheduling that completes, on average, the jobs for a 12\% earlier than the normal scenario.

This test reveals that so far, there is no need of using an asynchronous scheduling.
Hence, the rest of the experiments will exclusively use the synchronous mode.

\subsection{Heterogeneous Workloads} 

\begin{figure}%[htp]
\centering
  \includegraphics[clip,width=0.75\columnwidth, trim={2.8cm 4.75cm 2.8cm 4.3cm}]{images/heterExecTime.pdf}
\caption{Execution times of workloads of 100 jobs with different rates of flexible (Showing the top of the chart, Y axis is not starting in 0).}\label{fig:heterExecTime}
\end{figure}

In this benchmark we mixed flexible and fixed jobs in the same workload in order to study their interaction.
The workloads were composed of 100 jobs and the percentage of flexible jobs determined the probability of a job being flexible.
We raised the ratio of flexible jobs between 0\% and 100\% in steps of 25\%.
Figure~\ref{fig:heterExecTime} depicts the execution times for these configurations.
In general, we can appreciate that the execution time decreases as the ratio of flexible jobs grows.
The results show a 10\%-gain with only a 50\%-rate of flexible jobs, and up to a 12\%-improvement when all of them are flexible.

\subsection{Checking Period Inhibitor in Micro-steps Applications}

\begin{figure}%[htp]
\centering
  \includegraphics[clip,width=\columnwidth, trim={2.8cm 10.1cm 1.95cm 11.35cm}]{images/schedPeriodSec.pdf}
\caption{Execution time for the different inhibition periods (bars) and the gain respect the fixed workload (percentage on the right of the bars).}\label{fig:schedPeriodSec}
\end{figure}

For this test we reduced the time step in the model to an average of 2 seconds in order to investigate the importance of the 
overhead incurred by the scheduling process.
Again, we generated workloads with a different number of jobs and executed them as both fixed and flexible workloads.
For the flexible workloads, we enabled the \textit{checking inhibitor} (see Section~\ref{subsubsec:dmr}) to prevent that each iteration triggers a check.
Figure~\ref{fig:schedPeriodSec} depicts the variation of malleability for a fixed execution.
The group at the top (``Flexible''), represents an execution without the \textit{checking inhibitor} mechanism.
The rest of the groups in the chart (bellow ``flexible''), show the execution time when configuring the inhibitor period to: 2, 5, 10 and 20 seconds (from top to bottom).
The conclusion is that this gain is virtually negligible or even negative in some cases.
Hence, enabling periods of \textit{checking inhibition} can avoid a burst of communications between the runtime and the RMS, reducing the overhead.
In this particular example, setting a period of 5 seconds between scheduling, not only offers better results than the fixed workload, but also outperforms a simple flexible workload. 


%% \subsection{Statistics and metrics}
\subsection{Reconfiguration Scheduling Performance Evaluation}
To conclude this section, we present a thorough analysis of the overhead of using our framework to enable malleability.
For this purpose, we used the FS application configured to perform 2 steps and to transfer 1~GB of data during the reconfiguration.
The idea is that each job executes an iteration, then it contacts with the RMS and resumes the execution in the second step, with the new configuration of processes.

Figure~\ref{fig:reconfTimes} shows the average time of 10 executions for each reconfiguration.
On the left (a) we can see the times taken by the RMS to determine an action (scheduling time).
From top to bottom, the first half of the chart depicts the expansions, while the second half, the shrinks.
The chart reveals a slight increment in the scheduling time when more nodes are involved in the process.

Chart in Figure~\ref{fig:reconfTimes}(b) shows the time needed to perform the transfers among processes between communicators.
There can be appreciated two interesting behaviors: 
\begin{itemize}
 \item The more processes involved in the reconfiguration, the shorter resize time.
That is why the chunks of data are smaller and the time needed to transfer them concurrently is lower (compare the time between 1 to 2 and 64 to 32 processes).
 \item Shrinks involve much more synchronization among processes and the greater the difference in the number of processes is, the more time is needed to synchronize all of them.
\end{itemize}

\begin{figure}%[ht]
\subfloat[Scheduling  time.]{%
  \includegraphics[clip,width=0.5\columnwidth,trim={4.5cm 2.5cm 6.5cm 2.5cm}]{images/studySchedTimes.pdf}\label{subfig:schedTimes}
}
\subfloat[Resize time.]{%
  \includegraphics[clip,width=0.5\columnwidth,trim={4.5cm 2.5cm 6.5cm 2.5cm}]{images/studyResizTimes.pdf}\label{subfig:resizTimes}
}
\caption{Time needed to reconfigure from/to processes.}\label{fig:reconfTimes}
\end{figure}

 \begin{table}
 \caption{Analysis of the actions taken by the DMR API in a 400-job workload.}
 \label{tab:actions}
 \centering
 \resizebox{\linewidth}{!}{%
 \begin{tabular}{cccc} 
 %& & \multicolumn{2}{ c| }{200 jobs} \\ \cline{3-4}
 & & Synchronous & Asynchronous\\ \toprule
 \multicolumn{1}{ c }{\multirow{4}{*}{\parbox{1.5cm}{None Action}}} &
 \multicolumn{1}{ c }{Minimum Time (s)} & 0.0010 & 0.0003\\
 \multicolumn{1}{ c  }{}                        &
 \multicolumn{1}{ c }{Maximum Time (s)} & 0.2078 & 0.1140\\
 \multicolumn{1}{ c  }{}                        &
 \multicolumn{1}{ c }{Average Time (s)} & 0.0094 & 0.0137\\
 \multicolumn{1}{ c  }{}                        &
 \multicolumn{1}{ c }{Standard Deviation (s)} & 0.0102 & 0.0112\\ \cmidrule{2-4}

 \multicolumn{1}{c}{\multirow{6}{*}{\parbox{1.5cm}{Action Expand}}} &
 \multicolumn{1}{c}{Quantity} & 50 & 107\\
 \multicolumn{1}{c}{}                        &
 \multicolumn{1}{c}{Actions/Job} & 0.125 & 0.267\\
 \multicolumn{1}{c}{}                        &
 \multicolumn{1}{c}{Minimum Time (s)} & 0.367 & 0.366\\
 \multicolumn{1}{c}{}                        &
 \multicolumn{1}{c}{Maximum Time (s)} & 0.530 & 40.418\\
 \multicolumn{1}{c }{}                        &
 \multicolumn{1}{c}{Average Time (s)} & 0.423 & 8.820\\
 \multicolumn{1}{c }{}                        &
 \multicolumn{1}{c}{Standard Deviation (s)} & 0.146 & 12.688\\ \cmidrule{2-4}
 
 \multicolumn{1}{c}{\multirow{6}{*}{\parbox{1.5cm}{Action Shrink}}} &
 \multicolumn{1}{c}{Quantity} & 194 & 303\\
 \multicolumn{1}{c}{}                        &
 \multicolumn{1}{c}{Actions/Job} & 0.485 & 0.757\\
 \multicolumn{1}{c}{}                        &
 \multicolumn{1}{c}{Minimum Time (s)} & 0.233 & 0.334\\
 \multicolumn{1}{c}{}                        &
 \multicolumn{1}{c}{Maximum Time (s)} & 0.541 & 0.555\\
 \multicolumn{1}{c}{}                        &
 \multicolumn{1}{c}{Average Time (s)} & 0.425 & 0.422\\
 \multicolumn{1}{c}{}                        &
 \multicolumn{1}{c}{Standard Deviation (s)} & 0.498 & 0.049\\ \bottomrule
 \end{tabular}}
 \end{table}
 
 We also have studied the overhead in a real workload execution, for instance,  Table~\ref{tab:actions} reports the statistics collected for a 400-job workload.
 The table is divided in three parts and shows the amount of actions taken and their execution time during the workload execution in both synchronous and asynchronous scheduling.
 
 When no action is performed, the time to decide is virtually null (average time and standard deviation of ``none action'').
 The time increases when the RMS takes an action because of the scheduling itself and the operations of reconfiguration performed by the runtime. 
 
 The first two rows of the second and the third part, give information about how many reconfigurations are scheduled per workload and per job.
 We can see that the synchronous version schedules fewer reconfigurations and not all this jobs are expected to be resized.
 Moreover, since we are processing workloads with many queued jobs, running jobs are likely to be shrunk in favor of the pending. 
 
 The table also demonstrates the negative effect of a timeout during an expansion.
 This effect is shown in the asynchronous scheduling column with the ``maximum'', ``average'' and ``standard deviation'' values.
 In addition to the maximum time taken by the runtime to assert the expanding operation, these timeouts reveal a non-negligible dispersion in the duration values for the ``expand'' action.
 In fact, having such a high standard deviation turns the average time little representative.
 



==> text/exp-results.tex <==
\section{Experimental Results}
\label{sec:results}

\subsection{Testbed}
For the experiments, we have generated workloads of different sizes, configuring the job submissions to the queue at their best performance.

We first evaluate the individual scalability of the three real applications.
%Figure~\ref{fig:apps-scal} depicts the behavior of each application.
These tests identify two parallel behaviors:
\begin{itemize}
 \item High scalability (CG and Jacobi).
 In this case both applications have a similar behavior, with the highest speed-up attained for 32 processes.
 However, from 8 processes on, the difference gain between tests drops below 10\%, so we consider 8 processes as a ``sweet configuration spot'' for these two applications.
 \item Constant performance (N-body).
 In contrast, this application reaches its maximum performance for 16 processes.
 However, in this case, the gain does not exceed 10\% with respect to the sequential run, so a single process is considered as the ``sweet spot''. 
\end{itemize}

From the perspective of computational cost, CG and Jacobi comprise ``short'' iterations that complete in less than 2 seconds, while N-body executes costly iterations, in the scale of minutes.
For this reason, for CG and Jacobi we enabled the \textit{scheduling period inhibitor} featured by the runtime,  in order to reduce the amount of communications with the RMS.

Table~\ref{tab:apps-conf} displays the configuration employed in the experimentation.
The job submission of each application is launched with its ``maximum'' value, reflecting the user-preferred scenario of a fast execution. 
Each workload is composed of a set of randomly-sorted jobs (with a fixed seed) which instantiate one of the three real applications (33\% of jobs of each application class).
Furthermore, the inter-arrival time among submissions is generated using the statistical model proposed by Feitelson~\cite{Feitelson1996}, which characterizes rigid jobs based on observations from logs of actual cluster workloads.

\subsection{Results}
Figure~\ref{fig:exps} depicts the execution time of each workload size comparing both configuration options: fixed and flexible.
The labels at the end of the ``flexible'' bars report the gain compared with the fixed version.
Table~\ref{tab:summary} details the measures extracted from the executions.
In the first column, we compare the average resource utilization for fixed and flexible workloads.
This rate corresponds to the average time when a node has been allocated by a job compared to the workload completion time.
These results indicate that the flexible workloads reduce the allocation of nodes around 30\%, offering more possibilities for queued jobs. 

% \begin{figure}%[ht]
% \subfloat[Workloads execution times (bars) and the gain of flexible workloads (bar labels).]{%
%   \includegraphics[clip,width=0.5\columnwidth, trim={2.1cm 10cm 1.9cm 11.35cm}]{images/experimentTimes.pdf}\label{fig:exps}
% }
% \subfloat[Average waiting time for all the jobs of each workload (bars) and the gain of flexible workloads (bar labels).]{%
%   \includegraphics[clip,width=0.5\columnwidth,trim={2.1cm 10cm 1.9cm 11.35cm}]{images/waitingTimes.pdf}\label{fig:waits}
% }
% \caption{.}\label{fig:reconfTimes}
% \end{figure}

\begin{figure}%[htp]
\centering
  \includegraphics[clip,width=0.9\columnwidth, trim={2.1cm 10cm 1.9cm 11.35cm}]{images/experimentTimes.pdf}
      %\vspace{-0.5cm}
\caption{Workloads execution times (bars) and the gain of flexible workloads (bar labels).}\label{fig:exps}
  %\vspace{-0.4cm}
\end{figure}

The second column of Table~\ref{tab:summary} shows the average waiting time of the jobs for each workload.
These times are illustrated in Figure~\ref{fig:waits}, together with the gain rate for flexible workloads.
The reduction around 60\% makes the job waiting time a crucial measure to keep in mind from the perspective of throughput.
In fact, this time is responsible for the reduction in the workload execution time.

\begin{figure}%[htp]
\centering
  \includegraphics[clip,width=0.9\columnwidth, trim={2.1cm 10cm 1.9cm 11.35cm}]{images/waitingTimes.pdf}
    %\vspace{-0.5cm}
\caption{Average waiting time for all the jobs of each workload (bars) and the gain of flexible workloads (bar labels).}\label{fig:waits}
\end{figure}

The last two columns of Table~\ref{tab:summary} present two more aggregated measures of all the jobs in the workload:
The first one is the average execution time;
the second is this execution time plus the waiting time of the job, referred to as completion time.
%The last two rows of Table~\ref{tab:summary} present the average execution and the completion (the waiting time plus the execution) time of all the jobs in the workload
The experiments show that jobs in the flexible workload are affected by the scale-down of their number of processes.
However, this is compensated by the waiting time which benefits the completion time.

\begin{table}
\caption{Summary of the averaged measures from all the workloads.}
\label{tab:summary}
\centering 
%\resizebox{\linewidth}{!}{
\begin{tabular}{ccllll}
\toprule
\#Jobs & Version & \pbox{2cm}{Resource utilization rate} & \pbox{2cm}{Job\\waiting time} & \pbox{2cm}{Job\\execution time} & \pbox{2cm}{Job\\completion time}\\ \midrule
\multirow{2}{*}{50-job} & Fixed & 98.71 \% & 4115.02 s. &  620.26 s. & 4735.28 s.\\
 & Flexible & 68.67 \% & 1359.92 s. & 900.3 s. & 2260.22 s.\\
\multirow{2}{*}{100-job} & Fixed & 97.39 \%&9750.34 s.& 586.64 s.&10336.98 s.\\
 & Flexible & 71.91 \%&2990.6 s.&858.16 s.&3848.76 s.\\
 \multirow{2}{*}{200-job} & Fixed & 98.38 \%&17466.2 s.&520.58 s.&17986.78 s.\\
 & Flexible & 73.54 \%&6856.8 s.&825.88 s.&7676.67 s.\\
 \multirow{2}{*}{400-job} & Fixed & 98.38 \%& 31788.39 s.&532.14 s.&32320.53 s.\\
 & Flexible & 73.54 \%&13861.03 s.& 843.19 s..& 14704.22 s.\\
\bottomrule
\end{tabular}%}
\end{table}

In order to understand the events during a workload execution, we have chosen the smallest workload to generate detailed charts and offer an in-depth analysis.

The top and the bottom plots in Figure~\ref{fig:alloc} represent the evolution in time of the allocated resources and the number of completed jobs.
It also shows the number of running jobs for fixed and flexible workloads (blue and red lines respectively).
The figures demonstrate that the flexible workload utilizes fewer resources; furthermore, there are more jobs running concurrently (top chart).
For both configurations, jobs are launched with the ``sweet spot'' number of processes; the fixed jobs obviously do not vary the amount of assigned resources, while in the flexible configuration, they are scaled-down as soon as possible.
This explains the reduction on the  utilization resources.
For instance, in the second half of the flexible shape in Figure~\ref{fig:alloc} (marked area), we find a repetitive pattern in which there are 5 jobs in execution which allocate 40 nodes.
The next eligible job pending in the queue needs 32 nodes to start.
Therefore, unless one of the running jobs finishes, the pending job will not start and the allocation rate will not be higher.
When a job eventually finishes and releases 8 nodes, the scheduler initiates the job requesting 32 nodes.
Now, the allocated nodes are 64 (the green peaks in the chart); however, as the job prefers 8 processes, it will be scaled-down.
 
At the beginning of the trace in the bottom of Figure~\ref{fig:alloc}, the throughput of the fixed workload is higher, but this occurs because the first jobs are completed earlier (they have been launched with the best-performance number of processes).
Meanwhile, in the flexible workload, many jobs are initiated (blue line) and, as soon as they start to finish, the throughput experiences a boost.

\begin{figure}%[ht]
\centering
\begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[clip,width=0.75\columnwidth]{images/wl50-both.png}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[black,thick,rounded corners] (0.315,0.97) rectangle (0.5,0.555);
    \end{scope}   
\end{tikzpicture}
  \caption{Evolution in time for the 50-job workload. Blue and Red lines represent the running jobs for fixed and flexible policies.}\label{fig:alloc}
\end{figure}

Figure~\ref{fig:timesApps} depicts the execution and waiting time of each job grouped by application.
The execution time (top row of charts) increases in the flexible workload for all the cases.
As we explained before, we are shrinking jobs as soon as they are initiated to their preferred value.
It implies a decrease in the performance because the lack of resources.
However, there is a job that leverages the benefits of an expansion.
Last Jacobi job experiences a drop in its execution time, since it has been expanded thanks to completed jobs have released their resources.

The row of charts at the bottom compares the waiting time of all the jobs for their fixed and flexible versions.
At the beginning there is no remarkable difference in the waiting time of both versions, however,
the incoming of new jobs does not stop and resources remain allocated for the running jobs in the fixed workload. The RMS cannot provide the means for draining faster the queue.
For this reason, queued jobs in the fixed workload, experience a dramatic delay in their initiation.

That difference in the initiation is crucial for the completion time of the job, as it is shown in Figure~\ref{fig:diffTimesApps}.
This Figure represents the difference in execution, waiting and completion time for each job grouped by application.
Again, the execution time remains bellow zero what means that the difference is negative and the flexible workload performs slower.
Nevertheless, this small drawback is highly compensated by the waiting time.
As can be seen, completion difference time shows a heavy dependency on the waiting time,
making it the main responsible for reducing the individual completion time, and in turn, the high throughput obtained in the experiments.

\begin{figure}%[ht]
\centering
  \includegraphics[clip,width=0.75\columnwidth]{images/timesApps.pdf}
  \caption{Execution (top) and waiting (bottom) times of each job grouped by applications (columns).}\label{fig:timesApps}
    %\vspace{-0.5cm}
\end{figure}

\begin{figure}%[ht]
\centering
  \includegraphics[clip,width=0.75\columnwidth]{images/diffTimesApps.pdf}
  \caption{Time difference for each job of their completion, execution and waiting time.}\label{fig:diffTimesApps}
    %\vspace{-0.5cm}
\end{figure}




==> text/exp-setup.tex <==
\section{Experimental Setup}
\label{sec:setup}
%In this section we present the HPC facility tdescribe the job reconfiguration policy;
%we also present the workload generation and the job configuration;
%finally, the behavior of the framework is studied in terms of throughput, resource utilization and waiting, execution and completion job times.

\subsection{Platform}
Our evaluation was performed on the Marenostrum Supercomputer at {\em Barcelona Supercomputing Center}.
Each compute node in this facility is equipped with two 8-core Intel Xeon E5-2670 processors running at 2.6~GHz with 128~GB of RAM.
The nodes are connected via an InfiniBand Mellanox FDR10 network.
For the software stack we used MPICH 3.2, OmpSs 15.06, and Slurm 15.08. 

Slurm was configured with the \textit{backfill} job scheduling policy.
Furthermore, we also enabled job priorities with the policy \textit{multifactor}.
Both were configured with default values.

\subsection{Flexible Applications}
For our experimentation we used one synthetic and three real applications, described below:

\subsubsection{Flexible Sleep (FS)}
This iterative synthetic application performs a \textit{sleep} in each step (iteration).
The time of the step depends on the number of processes deployed in that iteration, so if the job is resized, the sleep time is modified assuming perfect linear scalability.
%The time of the sleep is determined by the model (\texttt{runtime} parameter) and is set depending on the \texttt{job size} (number of nodes).
Apart from the \textit{sleep} that simulates the computation time, the application also manages an array of doubles, distributed among the ranks. 
This array conforms the data-dependency for OmpSs, redistributed in each reconfiguration.

\subsubsection{Conjugate Gradient (CG)}
The CG method{\footnote{\url{https://en.wikipedia.org/wiki/Conjugate_gradient_method}}} is an iterative algorithm for the numerical solution of sparse systems of linear equations that produces a solution after a finite number of steps.
For our experimentation the method will perform a specific number of iterations in order to have control of the execution time.
%in order to have a strict control of the execution.
%However, we will configure the applications preventing them from converging.
%Instead, they will perform an arbitrary number of iterations in order to have control of the number of executions.

The data of the application propagated in each iteration step of CG is constrained to a matrix flat-stored and four vectors.
This version is implemented using OpenMP+MPI, and each MPI process works on a block of rows of the matrix and the corresponding elements from the vectors.
The local matrix-vector products are parallelized with OpenMP.

We have applied our OmpSs-based extensions in order to ease the creation of new processes while maintaining the data dependencies after the resizing procedure.
The five data structures in CG conform the data-dependencies between iterations in the OmpSs programming model, and they are redistributed when a rescaling is necessary.

During a resize, the data in the matrix and vectors must be redistributed according to the new number of MPI processes.

\subsubsection{Jacobi}
The Jacobi method\footnote{\url{https://en.wikipedia.org/wiki/Jacobi_method}} is an iterative and embarrassingly-parallel algorithm for the solution of a system of linear equations.

Our OpenMP+MPI version of this solver is based on the implementation presented in~\cite{Jajaga2012}.
The program layout is similar to the CG implementation.
In this application, we also have a flat matrix, but only two vectors.
These three structures conform the data-dependencies for OmpSs and they are all distributed among the processes.

\subsubsection{N-body}
\label{subsec:nbody}
The N-body problem\footnote{\url{https://en.wikipedia.org/wiki/N-body_problem}} simulates the individual motions of a group of objects interacting with each other by means of a given force.

We have used an OmpSs+MPI version of this simulator where each process stores a subset of particles, while the intra-node parallelism is exploited by OmpSs.

The amount of work of N-body per iteration is considerably larger than that present in the remaining two real applications described in this section.
Apart from computing the position and forces of its own particles, each process exchanges its local subset of particles with the other processes.
At the end of the iteration, all the processes have worked with the whole set of particles.

The data-dependency in this particular case is dictated by an array of particles with information about position, velocity, mass and weight.
This array is split or merged when an scale-up or down is respectively scheduled.


\subsection{Workload Configuration}
\label{subsec:workload}
The workloads were generated using the statistical model proposed
by Feitelson~\cite{Feitelson1996}, which characterizes rigid jobs based on observations from logs of actual cluster workloads. 
These include the distribution of job sizes in terms of number of processors, the correlation of runtime with parallelism, and the number of repeated runs.
Among others, we found four customizable parameters to be especially relevant:
\begin{itemize}
	\item \texttt{Jobs}: Number of jobs to be launched.
	\item \texttt{Job size}: Number of nodes determined by a complex discrete distribution.
	\item \texttt{Runtime}: Fixed following a hyperexponential distribution based on the \texttt{job size}.
	\item \texttt{Arrival}: Inter-arrival times of jobs modeled using a Poisson distribution.  
\end{itemize}
For every job the \texttt{shrink-expand factor} was set to 2.

